DiffusionNAG: Predictor-guided Neural Architecture Generation with Diffusion Models

Existing NAS methods suffer from either an excessive amount of time for repetitive sampling and training of many task-irrelevant architectures. To tackle such limitations of existing NAS methods, we propose a paradigm shift from NAS to a novel conditional Neural Architecture Generation (NAG) framework based on diffusion models, dubbed DiffusionNAG. Specifically, we consider the neural architectures as directed graphs and propose a graph diffusion model for generating them. Moreover, with the guidance of parameterized predictors, DiffusionNAG can flexibly generate task-optimal architectures with the desired properties for diverse tasks, by sampling from a region that is more likely to satisfy the properties. This conditional NAG scheme is significantly more efficient than previous NAS schemes which sample the architectures and filter them using the property predictors. We validate the effectiveness of DiffusionNAG through extensive experiments in two predictor-based NAS scenarios: Transferable NAS and Bayesian Optimization (BO)-based NAS. DiffusionNAG achieves superior performance with speedups of up to 35 times when compared to the baselines on Transferable NAS benchmarks. Furthermore, when integrated into a BO-based algorithm, DiffusionNAG outperforms existing BO-based NAS approaches, particularly in the large MobileNetV3 search space on the ImageNet 1K dataset. Code is available at https://github.com/CownowAn/DiffusionNAG.

==> 5_experiment_old.tex <==
\section{Experiment}

In this section, we present an extensive experimental validation of our proposed score-based neural architecture generation framework. In~\cref{sec:exp-guided}, we validate and analyze the effectiveness of our surrogate model in guiding the sampling process towards the desired architecture. In Section~\ref{sec:exp-multi-guided}, we verify the ability of our framework to efficiently sample optimal architectures within a given resource budget. Finally, in Section~\ref{sec:exp-metanas}, we compare our proposed framework to various neural architecture search methods.

\subsection{Experiment Setup}
\label{sec:experiment_setup}
\vspace{-0.05in}

\textbf{Search Space}
In~\cref{sec:exp-guided},~\cref{sec:exp-multi-guided}, and~\cref{sec:exp-metanas}, we evaluate our proposed score-based neural architecture generation framework using the NAS-Bench-201 search space benchmark~\citep{dong2020nasbench201}. The NAS-Bench-201 search space is composed of cell-based neural architectures, where each cell is represented as a Directed Acyclic Graph (DAG) consisting of 4 nodes and 6 edge connections. For each edge connection, NAS models select one of the 5 operation candidates, among $\{zerorize,\ skip-connect,\ 1\times1\ conv,\ 3\times3\ conv,\ 3\times3\ avg\ pool\}$. 

\textbf{Source Database}
% In~\cref{sec:exp-guided} and~\cref{sec:exp-multi-guided}, we use the (architecture, accuracy, latency) pairs in NAS-Bench-201 benchmark~\citep{dong2020nasbench201} to train our auxiliary predictor network which is trained for each dataset.
% We collect 10,000/15,625 pairs for training the predictor and the rest were used as a validation set.
In~\cref{sec:exp-guided} and~\cref{sec:exp-multi-guided}, we use the (architecture, accuracy, latency) pairs from the NAS-Bench-201 benchmark~\citep{dong2020nasbench201} to train our auxiliary predictor network. In these sections, training is performed separately for each dataset. Also, we collect 10,000/15,625 pairs for training the predictor network, and the remaining samples were used as a validation set. This allows us to train a predictor network that can accurately guide the sampling process in the direction we want to generate.
In~\cref{sec:exp-metanas}, following~\citet{lee2021rapid}, we collect multiple tasks where each task consists of (dataset, architecture, accuracy, latency) to train our auxiliary time-dependent meta-predictor network. As described in~\citet{lee2021rapid}, the dataset of each task is composed of multiple sub-sets of ImageNet-1K~\citep{imagenet_cvpr09} that are randomly sampled 20 classes 
% with an average of 26K images for each sub-sets 
and all images are downsampled by 32 × 32 size. 
We collect 4,230 meta-training tasks for our time-dependent meta-predictor and 400 meta-validation tasks for them, respectively same as~\citet{lee2021rapid}.
After training the time-dependent meta-predictor, we validate the effectiveness of our model by searching for architectures on 6 benchmark datasets in~\cref{sec:exp-metanas}. 

\textbf{Diffusion Model} In our score-based neural architecture generation framework, we use the VP SDE~\citep{song2021scorebased} numerical SDE solver for the forward and reverse diffusion processes. The score-based model is trained in an unconditional manner and we generate samples using the Langevin MCMC algorithm with 1000 discretization steps. This allows us to efficiently sample high-performing architectures while ensuring that the generated samples are distributed according to the learned score-based model.

% \subsection{prior validity, uniqueness and novelty}\label{sec:exp-predictor}
% \subsection{Auxiliary Predictor Network}\label{sec:exp-predictor}
% To achieve the desired objective in the generation of neural architectures, as discussed in~\cref{sec:method-guided}, we exploit an auxiliary predictor network. To train this network, we utilize data with a time-dependent noise scale applied, $(\bm{A}_t, y)$. And the training objective is a simple sum of MSE losses sampled at different scales. We provide a plot to show the correlation coefficient of this auxiliary prediction network over noise scales.

\subsection{Controllable Neural Architectures Generation}\label{sec:exp-guided}
\input{Figure_Tex/single_guided/cifar10/acc.tex}
\input{Figure_Tex/single_guided/cifar10/latency_10}
\input{Figure_Tex/single_guided/cifar10/latency_15}
\input{Figure_Tex/single_guided/cifar10/flops_10}
\input{Figure_Tex/single_guided/cifar10/flops_50}
\input{Figure_Tex/single_guided/cifar10/params_0.1}
\input{Figure_Tex/single_guided/cifar10/params_0.5}
% \input{Figure_Tex/single_guided/scatter/cifar10/latency.tex}
% \input{Figure_Tex/single_guided/box/cifar10}
% We first validate and analyze our score-based neural architecture generation framework in terms of whether the auxiliary predictor model can guide the sampling process in the direction we want to generate.
% To achieve the desired objective in the generation of neural architectures, as discussed in~\cref{sec:method-guided}, we exploit an auxiliary predictor network. To train this network, we utilize data with a time-dependent noise scale applied, $(\bm{A}_t, y)$. And the training objective is a simple sum of MSE losses sampled at different scales. We provide a plot to show the correlation coefficient of this auxiliary prediction network over noise scales.
% In order to validate our method, we evaluate 1,000 generated neural architectures by measuring \textbf{Top 1\% property} that is the average of top 1\% target property values such as accuracy or latency. 
In this section, we validate and analyze our score-based neural architecture generation framework in terms of whether the auxiliary predictor model can effectively guide the sampling process towards the desired architectures.
As discussed in Section~\ref{sec:method-guided}, we exploit an auxiliary predictor network to achieve this objective. The predictor network is trained on data with a time-dependent noise scale applied, $(\bm{A}_t, y)$, and the training objective is a simple sum of MSE losses sampled at different noise scales. 
% We provide a plot to show the correlation coefficient of this auxiliary prediction network over noise scales.
After training the auxiliary time-dependent predictor network, we evaluate 1,000 generated neural architectures by measuring the \textbf{Top 1\% property}. This is defined as the average of the top 1\% target property values such as accuracy or latency.
This allows us to quantify the effectiveness of our proposed score-based neural architecture generation framework in generating architectures that possess the desired properties.

In~\cref{tbl:top_dist}, \textbf{No Gui.} corresponds to the situation where there is no guide in the reverse sampling process. And \textbf{ACC-Gui.} means that the sampling process is guided in the direction of maximizing accuracy which corresponds to the situation when the $w = 0$ in~\cref{eq:mult-obj}, while \textbf{LAT-Gui.} means that our diffusion generator is guided in the direction of minimizing latency without considering accuracy.
Further, we also measured the number of unique neural architectures among the sampled neural architectures which is referred to as \textbf{Uniqueness}.
% Further, we also measured the number of neural architectures that need to be sampled to obtain target properties, which is referred to as \textbf{Number of samples required}.
% plot 추가
% Also, We visualize the distribution of the generated neural architectures via two-dimensional uniform manifold approximation and projection (UMAP) in Figure 3 (Left). We observe that 
% deviation from the training dataset to be controllable with the hyperparameter 
% It was confirmed that guided sampling was working well in the direction to be maximized. In addition, it was also confirmed that as the guidance scale value increases, sampling is guided with a narrow distribution (small uniqueness) closer to the desired property.

Our experimental results in~\cref{tbl:top_dist} confirm that the guided sampling works well in the direction of the property to be maximized. Furthermore, as the guidance scale value increases, the sampling is guided with a narrow distribution (small uniqueness in~\cref{tbl:uniqueness}) closer to the desired property. This confirms that our proposed auxiliary predictor network effectively guides the sampling process towards architectures with the desired properties.

\subsection{Single-objective guided sampling}\label{sec:exp-single-guided}
\input{Figure_Tex/SO_BO/NB201/C10}
\input{Figure_Tex/SO_BO/NB201/C100}
\subsection{Multi-objective guided sampling}\label{sec:exp-multi-guided}
% \input{Figure_Tex/fig_multi_guided.tex}
 In real-world scenarios, rather than considering only single objectives such as accuracy or latency, we are more interested in finding multiple Pareto-optimal~\citep{deb2014multi} solutions in neural architecture search. And as described in~\cref{sec:method-multiobj}, our diffusion sampler can be controlled to generate a neural architecture with maximum performance within a resource budget using the objective in~\cref{eq:mult-obj}.

\subsection{Transfer NAS}\label{sec:exp-metanas}
\input{Table/tbl_main_nasbench201.tex}
% \input{Figure_Tex/fig_meta_nas.tex}

==> Algo/pc_sampler.tex <==
\begin{figure}[t!]
\vspace{-0.2in}
\centering
\begin{minipage}{0.7\linewidth}
\centering
\begin{algorithm}[H]
    \small
    \caption{ PC Sampler for DiffusionNAG }\label{alg:sampler}
        \textbf{Input:} Trained model $\bm{s}_{\bm{\theta}^*}$, number of sampling steps $T$, number of correction steps per prediction $M$, diffusion step size $\mathrm{d}t$, score-to-noise ratio $r$, scaling coefficient $\epsilon_s$ \\
        \textbf{Output:} Sampled graph $\bm{G}$
    \begin{algorithmic}[1]
        \STATE Sample number of nodes $N$ from the training set.
        \STATE $\bm{G}_0\sim \mathcal{N}(0,\mathbf{I}_N)$
        \COMMENT{Start from noise}
        \STATE $t\leftarrow 0$
        \FOR{$k=1$ \textbf{to} $K$}
            \STATE $\eta \leftarrow \alpha\sigma_t^2\bm{G}_{t} + \frac{\sigma_t^2}{v_t}\left(\frac{1}{u_t}\bm{s}_{\theta}(\bm{G}_{t},t) - \bm{G}_{t}\right)$
            \COMMENT{Compute drift}
            \STATE $\mathbf{w}\sim\mathcal{N}(0,\mathbf{I}_N)$ 
            \STATE $\tilde{\bm{G}_{t}}\leftarrow \eta\mathrm{d}t +  \sigma_t \sqrt{\delta t} \mathbf{w}$
            \COMMENT{Predictor: Euler-Maruyama}
            \FOR{$m=1$ \textbf{to} $M$}
                \STATE $\tilde{\eta} \leftarrow \alpha\tilde{\bm{G}_{t}} + \frac{1}{v_t}\left(\frac{1}{u_t}\bm{s}_{\theta}(\tilde{\bm{G}_{t}},t) - \tilde{\bm{G}_{t}}\right)$
                % \COMMENT{Compute the score}
                \STATE $\mathbf{w}\sim\mathcal{N}(0,\mathbf{I}_N)$ 
                \STATE $\epsilon \leftarrow 2\left(r\|\mathbf{w}\|_2/\|\tilde{\eta}\|_2  \right)^2$ 
                \COMMENT{Corrector step size}
                \STATE $\bm{G}_{t+\mathrm{d}t} \leftarrow \tilde{\bm{G}_{t}} + \tilde{\eta}\epsilon + \epsilon_s\sqrt{2\epsilon}\mathbf{w}$
                \COMMENT{Corrector: Langevin dynamic}
            \ENDFOR
            \STATE $t\leftarrow t+\mathrm{d}t$
        \ENDFOR
        \STATE $\bm{G}\leftarrow \texttt{quantize}(\bm{G}_t)$
        \COMMENT{quantize if necessary}
        \STATE \textbf{Return:} graph $\bm{G}$ 
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-0.1in}
\end{figure}



% \begin{figure}[ht]
% \vspace{-0.15in}
% \centering
% \begin{minipage}{1.0\textwidth}
% \begin{algorithm}[H]
%    \caption{\small Bayesian Optimization with DiffusionNAG}
%      \KwIn{Pre-trained score network $\bm{s}_{\bm{\theta}^*}$, search space $\mathcal{A}$, dataset $\mathcal{D}$, parameters $n_0$, $N$, $c$, function $h:\mathcal{A}\to \mathbb{R}$ returning validation accuracy of an architecture $\bm{A}\in\mathcal{A}$.}
%      Draw $n_0$ architectures $\bm{A}^{(1)}, \ldots, \bm{A}^{(n_0)}$ uniformly from the search space $\mathcal{A}$ and train them on $\mathcal{D}$ to construct $\bm{B}_{n_0}=\{(\bm{A}^{(1)}, h(\bm{A}^{(1)})), \ldots, (\bm{A}^{(n_0)}, h(\bm{A}^{(n_0)}) ) \}$. \\
%     \For{$n=n_0,\ldots, N-1$}{
%          Train an  ensemble of $M$ surrogate model $\{\hat{h}_{\psi_m}\}_{m=1}^M$ based on the current population $\bm{B}_n$: \\$\psi^*_m\in \argmin_{\psi_m} \sum_{i=1}^n 
%         \left( h(\bm{A}^{(i)}) - \hat{h}_{\psi_m}( \bm{A}^{(i)})\right)^2$ for $m=1,\ldots, M$. \\
%         $\hat{\mu}(\bm{A}^{(i)}) \coloneqq \frac{1}{M} \sum_{m=1}^M \hat{h}_{\psi^*_m}(\bm{A}^{(i)})$ \\
%         $\hat{\sigma}_{i}(\bm{A}^{(i)})\coloneqq \sqrt{\frac{\sum_{m=1}^M((\hat{h}_{\psi^*_m}(\bm{A}^{(i)})- \mu(\bm{A}^{(i)}))^2 }{M-1}}$ \\
%         $p(y| \bm{A}^{(i)};\mathcal{D})\coloneqq \mathcal{N}(y;\hat{\mu}((\bm{A}^{(i)})), \hat{\sigma}(\bm{A}^{(i)})^2)$. \\
        
%         \boxit{figred}{10}\tcc{Generate $c$ candidate architecture with the score network $\bm{s}_{\bm{\theta}^*}$.}
%         $S\leftarrow \emptyset$ \\
%         Minimize $\sum_{i=1}^n -\log p_\xi(y_i | \bm{A}^{(i)})$ w.r.t $\xi$, where $y_i = h(\bm{A}^{(i)})$. \\
%         \For{$i=1,\ldots, c$}{
%          Draw a random noise $\bm{A}^{(n+i)}_T$ from the prior distribution. \\
%         Generate architecture $\bm{A}^{(n+i)}$ with $\bm{s}_{\bm{\theta^*}}$ by the reverse process: \\
%         $d\bm{A}^{(n+i)}_t=\left\{\mathbf{f}_{t}(\bm{A}^{(n+i)}_t) - g_{t}^2 \Big[\bm{s}_{\bm{\theta}^*}(\bm{A}^{(n+i)}_t, t) + k_t {\nabla_{\bm{A}^{(n+i)}_t}\! \log p_\xi(y|\bm{A}^{(n+i)}_t)}\Big]\right\}\mathrm{d}\overbar{t}
%     + g_{t}\mathrm{d}\bar{\mathbf{w}}$
%         $S\leftarrow S \cup \{\bm{A}^{(n+i)}_0 \}$}
%         For each candidate architecture $\bm{A}\in S$, evaluate $\varphi(\bm{A})$ with $p(y| \bm{A}^{(i)};\mathcal{D})$. \\
%         Select architecture $\bm{A}^{(n+1)}$ which maximizes $\varphi(\bm{A})$. \\
%         Train architecture $\bm{A}^{(n+1)}$ to get the accuracy $h(\bm{A}^{(n+1)})$ and add it to the population $\bm{B}_n$:   $\bm{B}_{n+1}=\bm{B}_n\cup \{(\bm{A}^{(n+1)}, h(\bm{A}^{(n+1)}) ) \}$.
%     }
%     \KwOut{$\bm{A}^* =  \argmax_{n=1,\ldots,N}h(\bm{A}^{(n)})$}
% \label{algo:general-diffusion}
% \end{algorithm}
% \end{minipage}
% \vspace{-0.1in}
% \end{figure}


==> Algo/transfer_nag.tex <==
\begin{figure}[t!]
\vspace{-0.2in}
\centering
\begin{minipage}{0.9\linewidth}
\centering
\begin{algorithm}[H]
    \small
    \caption{ Symmetric Splitting for the System of SDEs (S4) }\label{alg:symmetric_splitting}
        \textbf{Input:} Score-based models $\bm{s}_{\theta,t}$ and $\bm{s}_{\phi,t}$, number of sampling steps $M$, step size $\delta t$, transition distributions $p_{st}(\cdot|\cdot)$ of the forward diffusion in Eq.~\eqref{eq:forward_diffusion}, Lagevin MCMC step size $\alpha$, scaling coefficient $\epsilon_s$ \\
        \textbf{Output:} $\bm{X}_0$, $\bm{A}_0$: the solution to Eq.~\eqref{eq:estimated_system_sdes}
    \begin{algorithmic}[1]
        \STATE $t=T$
        \STATE Sample from the prior distribution $\bm{X}_M,\!\bm{A}_M\sim p_T$
        \FOR{$m=M-1$ \textbf{to} $0$}
            \STATE $\bm{S}_{X} \leftarrow \bm{s}_{\theta,t}(\bm{X}_{m+1},\!\bm{A}_{m+1})$; \;\;
            $\bm{S}_A \leftarrow \bm{s}_{\phi,t}(\bm{X}_{m+1},\!\bm{A}_{m+1})$ \COMMENT{score computation step}
            \STATE $\bm{X}_{m+1}\leftarrow \bm{X}_{m+1} + \frac{\alpha}{2}\bm{S}_X + \epsilon_s \sqrt{\alpha}\bm{z}_X$; \;\; $\bm{z}_X\sim\mathcal{N}\left(\bm{0},\bm{I}_{X}\right)$ \COMMENT{correction step: $\bm{X}$}
            \STATE $\bm{A}_{m+1}\,\leftarrow \bm{A}_{m+1}\, + \frac{\alpha}{2}\bm{S}_A + \epsilon_s \sqrt{\alpha}\bm{z}_A$; \;\; $\bm{z}_A\sim\mathcal{N}\left(\bm{0},\bm{I}_{A}\right)$ \COMMENT{correction step: $\bm{A}$}
            \STATE $t' \leftarrow t - \delta t/2$
            \STATE $\tilde{\bm{X}}_{m}\sim p_{t,t'}(\tilde{\bm{X}}_{m}|\bm{X}_{m+1})$; \;\; $\tilde{\bm{A}}_{m}\sim p_{t,t'}(\tilde{\bm{A}}_{m}|\bm{A}_{m+1})$ \COMMENT{prediction step: action of $e^{\frac{\delta t}{2}\fop_{F}}$}
            \STATE $\tilde{\bm{X}}_{m}\leftarrow\tilde{\bm{X}}_{m} + g^2_{1,t}\bm{S}_{X}\delta t$; \;\; $\tilde{\bm{A}}_{m}\leftarrow\tilde{\bm{A}}_{m} + g^2_{2,t}\bm{S}_{A}\delta t$ \COMMENT{prediction step: action of $e^{\delta t\fop_{S}}\,\,$}
            \STATE $t\leftarrow t-\delta t$
            \STATE $\bm{X}_{m}\sim p_{t',t}(\bm{X}_{m}|\tilde{\bm{X}}_{m})$; \, $\bm{A}_{m}\sim p_{t',t}(\bm{A}_{m}|\tilde{\bm{A}}_{m})$ \COMMENT{prediction step: action of $e^{\frac{\delta t}{2}\fop_{F}}$}
        \ENDFOR
        \STATE \textbf{Return:} $\bm{X}_0$, $\bm{A}_0$ 
    \end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-0.2in}
\end{figure}

==> Figure_Tex/SO_BO/NB201/C10.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[EI]{
	\includegraphics[width=3.15cm]{Figure/SO_BO/NB201/C10/cifar10_ei.png}
	\label{fig:SO_BO_C10_ei_nb201}
	}
	\subfigure[TS]{
	\includegraphics[width=3.15cm]{Figure/SO_BO/NB201/C10/cifar10_ts.png}
	\label{fig:sSO_BO_C10_ts_nb201}
	}
        \subfigure[PI]{
	\includegraphics[width=3.15cm]{Figure/SO_BO/NB201/C10/cifar10_pi.png}
	\label{fig:SO_BO_C10_pi_nb201}
	}
        \subfigure[UCB]{
	\includegraphics[width=3.15cm]{Figure/SO_BO/NB201/C10/cifar10_ucb.png}
	\label{fig:SO_BO_C10_ucb_nb201}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Acquisition Function Optimization Strategy} We provide a pool of candidate neural architectures guided towards the direction of good performance using a trained model set.}
	\label{fig:SO_BO_C10_nb201}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/analysis/poor_arch.tex <==
\begin{wrapfigure}{r}{0.32\textwidth} 
 \vspace{-0.23in}
  \begin{center}
	\subfigure{
        \includegraphics[width=0.32\textwidth]{Figure/analysis/poor_arch/scatter_anal.png}
	\label{fig:cub_time}
	}
 \vspace{-0.25in}
 \caption{\small \textbf{Generated architectures with poor training set.}}
\label{fig:poor_arch}
  \end{center}
 \vspace{-0.2in}
\end{wrapfigure}


==> Figure_Tex/controllable_gen/controllable_gen.tex <==



% \begin{wrapfigure}{r}{0.25\textwidth} 
%  \vspace{-0.25in}
%   \begin{center}
%     \includegraphics[width=0.9\linewidth]{1_Figure_Raw/size_meta_training2.pdf}
%  \vspace{-0.1in}
% \caption{\small Effect of the meta-training pool size.}
% \label{fig:size_meta_train}
%   \end{center}
%  \vspace{-0.2in}
% \end{wrapfigure} 




\begin{wrapfigure}{r}{0.7\textwidth} 
    % \vspace{-0.05in}
	\centering
	\vspace{-0.25in}
	%\subfigure[]{
	% \includegraphics[width=4.5cm]{Figure/controllable_gen/acc/scatter.png}
	% \label{fig:controllable_acc}
	%}
	%\subfigure[]{
	\includegraphics[width=0.343\textwidth]{Figure/controllable_gen/latency/scatter.png}
	\label{fig:controllable_latency}
	%}
        %\subfigure[]{
	\includegraphics[width=0.343\textwidth]{Figure/controllable_gen/params/scatter.png}
	\label{fig:controllable_params}
	%}
	\vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} 
 % Neural architectures are generated in a way that \textbf{maximized} \textbf{accuracy}, guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $1000$.
     }
	\label{fig:controllabel_gen}
	\vspace{-0.1in}
\end{wrapfigure} 

% Target objective의 종류를 다르게 해가면서 우리 generative framework의 효력을 확인하였다.
% Accuracy Guide의 경우, accuracy가 maximize되는 방향으로 guided sampling을 했으며, Latency Guide와 #Params Guide의 경우, 각각의 target objective가 minimize되는 방향으로 guided sampling을 했다. 이 경우에 surrogate model은 1000개의 샘플로 학습되었다.


==> Figure_Tex/fig_concept_1.tex <==
\begin{figure*}[t]
    \small
    \centering
        \vspace{-0.05in}
	\centering
	\hfill
	\subfigure[Motivation 1]{
	\includegraphics[height=3.6cm]{Figure/fig_motivation_1.pdf}
	%\label{fig:concept1}
	}
	%\hfill
	\subfigure[Motivation 2]{
	\includegraphics[height=3.6cm]{Figure/fig_motivation_2.pdf}
	%\label{fig:concept1}
	%\label{fig:concept1}
	}
    % \vspace{-0.05in}
    % \includegraphics[width=0.98\textwidth]{Figure/fig_concept.pdf} 
    \vspace{-0.1in}
    \caption{\small \textbf{Score-based neural architecture generation framework} \small 
    }
    \label{fig:concept_1}
    \vspace{-0.15in}
\end{figure*}


==> Figure_Tex/fig_concept_2.tex <==
\begin{figure*}[t]
    \small
    \centering
    \vspace{-0.05in}
    \includegraphics[width=0.98\textwidth]{Figure/fig_concept.pdf} 
    \vspace{-0.1in}
    \caption{\small \textbf{Score-based neural architecture generation framework.} \small 
    Our proposed framework can generate an optimal neural architecture for a given dataset under user-defined multiple conditioning by using the gradient of meta-trained proxy predictors, ${\nabla_{\bm{A}_t}\!\ f(\tau, \bm{A}_t, t;\bm{\phi})}$ during the reverse time diffusion process. In other words, ours can tackle an important problem of generalization (transferability) of NAS models over realistic tasks involving accuracy, datasets, and resource budgets to
    be addressed for NAS to be truly practical in the real world.
    }
    \label{fig:concept_2}
    \vspace{-0.05in}
\end{figure*}


==> Figure_Tex/fig_meta_nas.tex <==
\begin{figure*}[t]
    \small
    \centering
    \vspace{-0.05in}
    \includegraphics[width=\columnwidth]{Figure/meta_nas/example_meta.png} 
    % \includegraphics{Figure/meta_nas/example_meta.png} 
    \vspace{-0.1in}
    \caption{\small \textbf{Task-guided Neural Architecture Generation} \small 
    ToDO
    }
    \label{fig:meta_nas}
    \vspace{-0.15in}
\end{figure*}


==> Figure_Tex/fig_multi_guided.tex <==
\begin{figure*}[t!]
    % \vspace{-0.05in}
    \centering
    \small
    \begin{tabular}{cccccc}
    \includegraphics[height=4cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=4cm] {Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=4cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}\\
    \vspace{-0.05in}
    (a) Accuracy &\hspace{-0.25in}
    (b) Latency
    \end{tabular}
    \vspace{-0.05in}
    \caption{\footnotesize \textbf{Pareto-optimal Curves with multi-objective guided neural architecture generation} TODO}
    \label{fig:multi_guided}
    \vspace{-0.1in}
\end{figure*}

==> Figure_Tex/fig_single_guided_ex.tex <==
\begin{figure*}[t!]
    % \vspace{-0.05in}
    \centering
    \small
    \begin{tabular}{cccccc}
    \includegraphics[height=2.5cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=2.5cm]
    {Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=2.5cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=2.5cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=2.5cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in}
    \includegraphics[height=2.5cm]{Figure/single_guided/example_acc_lat.png}&\hspace{-0.25in} 
    \\
    \vspace{-0.05in}
    (a) Accuracy &\hspace{-0.25in}
    (b) Latency
    \end{tabular}
    \vspace{-0.05in}
    \caption{\footnotesize \textbf{Controllable Neural Architecture Generation} TODO}
    \label{fig:single_guided}
    \vspace{-0.1in}
\end{figure*}

==> Figure_Tex/single_guided/cifar10/acc.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/acc/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_acc_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/acc/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_acc_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/acc/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_acc_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-acc_max_box.png}
	\label{fig:single_scatter_cifar10_acc_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in a way that \textbf{maximized} \textbf{accuracy}, guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$.}
	\label{fig:single_scatter_cifar10_acc}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/flops_10.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/10/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/10/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-flops_10.0_box.png}
	\label{fig:single_scatter_cifar10_flops_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of \textbf{FLOPs} become \textbf{10 (M)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$ and the FLOPs in NAS-Bench-201 are based on a $32 \times 32$ image size}
	\label{fig:single_scatter_cifar10_flops_10}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/flops_50.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/50/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_0.1}
	}
        \subfigure[Guide (0.5]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/flops/50/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_flops_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-flops_50.0_box.png}
	\label{fig:single_scatter_cifar10_flops_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of \textbf{FLOPs} become \textbf{50 (M)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$ and the FLOPs in NAS-Bench-201 are based on a $32 \times 32$ image size.}
	\label{fig:single_scatter_cifar10_flops_50}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/latency_10.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/10/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/10/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-latency_0.01_box.png}
	\label{fig:single_scatter_cifar10_latency_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of \textbf{latency} become \textbf{10 (ms)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$ and the latency in NAS-Bench-201 is computed by running each model on a single GPU (GeForce GTX 1080 Ti) with a batch size of $256$.}
	\label{fig:single_scatter_cifar10_latency_10}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/latency_15.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/15/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/latency/15/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_latency_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.0cm]{Figure/single_guided/box/cifar10/target-latency_0.015_box.png}
	\label{fig:single_scatter_cifar10_latency_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of \textbf{latency} become \textbf{15 (ms)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$ and the latency in NAS-Bench-201 is computed by running each model on a single GPU (GeForce GTX 1080 Ti) with a batch size of $256$.}
	\label{fig:single_scatter_latency_15}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/params_0.1.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/0.1/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/0.1/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-params_0.1_box.png}
	\label{fig:single_scatter_cifar10_params_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of \textbf{the number of parameters} become \textbf{0.1 (MB)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$.}
	\label{fig:single_scatter_cifar10_params_0.1}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided/cifar10/params_0.5.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/0.5/weight_x-r0.1-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_0.1}
	}
        \subfigure[Guide (0.5)]{
	\includegraphics[width=3.15cm]{Figure/single_guided/scatter/cifar10/params/0.5/weight_x-r0.5-filtered_G-F-text-F_scatter.png}
	\label{fig:single_scatter_cifar10_params_0.5}
	}
        \subfigure[Dist.]{
	\includegraphics[width=3.15cm]{Figure/single_guided/box/cifar10/target-params_0.5_box.png}
	\label{fig:single_scatter_cifar10_params_dist}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in such a way that the values of  \textbf{the number of parameters} become \textbf{0.5 (MB)} guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is $100$.}
	\label{fig:single_scatter_cifar10_params_0.5}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided_old/box/cifar10.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[Accuracy]{
	\includegraphics[width=5.0cm]{Figure/single_guided/box/cifar10/target-acc_box.png}
	\label{fig:single_box_cifar10_acc}
	}
	\subfigure[Latency]{
	\includegraphics[width=5.0cm]{Figure/single_guided/box/cifar10/target-latency_box.png}
	\label{fig:single_box_cifar10_latency}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Distribution of neural architectures with respect
to the guiding objective.}}
	\label{fig:single_box_cifar10}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided_old/scatter/cifar10/acc.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/no_guide_scatter.png}
	\label{fig:single_scatter_cifar10_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/acc/after_sp_weight_x-0.1_scatter.png}
	\label{fig:single_scatter_cifar10_acc_0.1}
	}
 %        \subfigure[Guide (0.5)]{
	% \includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/acc/after_sp_weight_x-0.5_scatter.png}
	% \label{fig:single_scatter_cifar10_acc_0.5}
	% }
        \subfigure[Guide (1.0)]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/acc/after_sp_weight_x-1.0_scatter.png}
	\label{fig:single_scatter_cifar10_acc_1.0}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.} Neural architectures are generated in a way that maximizes accuracy, guided by a noise-aware predictor network, $f(\cdot; \phi)$. The number of samples is 200.}
	\label{fig:single_scatter_cifar10_acc}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/single_guided_old/scatter/cifar10/latency.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\subfigure[No Guide]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/no_guide_scatter.png}
	\label{fig:single_scatter_cifar10_no_guide}
	}
	\subfigure[Guide (0.1)]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/latency/after_sp_weight_x-0.1_scatter.png}
	\label{fig:single_scatter_cifar10_latency_0.1}
	}
 %        \subfigure[Guide (0.5)]{
	% \includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/latency/after_sp_weight_x-0.5_scatter.png}
	% \label{fig:single_scatter_cifar10_latency_0.5}
	% }
        \subfigure[Guide (1.0)]{
	\includegraphics[width=4.2cm]{Figure/single_guided/scatter/cifar10/latency/after_sp_weight_x-1.0_scatter.png}
	\label{fig:single_scatter_cifar10_latency_1.0}
	}
	% \vspace{-0.15in}
	\caption{\small \textbf{Objective-controllable neural architectures generation.}}
	\label{fig:single_scatter_cifar10_latency}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/transfer_nas/mbv3.tex <==
\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	%\subfigure[]{
	\includegraphics[width=3.35cm]{Figure/transfer_nas/mbv3/main_mbv3_cifar10.pdf}
	\label{fig:transfer_nas_c10}
	%}
	%\subfigure[]{
	\includegraphics[width=3.35cm]{Figure/transfer_nas/mbv3/main_mbv3_cifar100.pdf}
	\label{fig:transfer_nas_c100}
	%}
        %\subfigure[]{
	\includegraphics[width=3.35cm]{Figure/transfer_nas/mbv3/main_mbv3_aircraft.pdf}
	\label{fig:transfer_nas_aircraft}
	%}
	% \vspace{-0.15in}
        \includegraphics[width=3.35cm]{Figure/transfer_nas/mbv3/main_mbv3_pets.pdf}
	\label{fig:transfer_nas_pets}
	%}
	%\subfigure[]{
	\caption{\small \textbf{: One-shot Generation Results}  }
	\label{fig:one_shot_gen_mbv3}
	\vspace{-0.1in}
\end{figure}

==> Figure_Tex/transfer_nas/nb201.tex <==
% \begin{figure}[t]
%     % \vspace{-0.05in}
% 	\centering
% 	\vspace{-0.1in}
% 	%\subfigure[]{
% 	\includegraphics[width=3.35cm]{Figure/transfer_nas/nb201/nb201_-_cifar10.png}
% 	\label{fig:transfer_nas_c10}
% 	%}
% 	%\subfigure[]{
% 	\includegraphics[width=3.35cm]{Figure/transfer_nas/nb201/nb201_-_cifar100.png}
% 	\label{fig:transfer_nas_c100}
% 	%}
%         %\subfigure[]{
% 	\includegraphics[width=3.35cm]{Figure/transfer_nas/nb201/nb201_-_aircraft.png}
% 	\label{fig:transfer_nas_aircraft}
% 	%}
% 	% \vspace{-0.15in}
%         \includegraphics[width=3.35cm]{Figure/transfer_nas/nb201/nb201_-_pets.png}
% 	\label{fig:transfer_nas_pets}
% 	%}
% 	%\subfigure[]{
% 	\caption{\small \textbf{: Comparison of DiffusionNAS to Various NAS methods.}  }
% 	\label{fig:transfer_nas_nb201}
% 	\vspace{-0.1in}
% \end{figure}

\begin{figure}[t]
    % \vspace{-0.05in}
	\centering
	\vspace{-0.1in}
	\includegraphics[width=1.0\textwidth]{Figure/transfer_nas/nb201/transfer_nas.png}
	\vspace{-0.2in}
	\caption{\small \textbf{Improving TransferNAS.} DiffusionNAG provides better quality neural architectures at the init phase, which results in improving the adaptation performance of TransferNAS. By conducting search adaptation on four unseen datasets with more samples, Diffusion-based TransferNAS outperforms other baselines significantly.} 	\label{fig:transfer_nas_nasbench201}

 
    \vspace{-0.2in}

\end{figure}

==> Figure_Tex/vis/mbv3.tex <==
\begin{figure}[t]
	\centering
	% \vspace{-0.1in}
         \subfigure[CIFAR-10]{
        	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_cifar10.pdf}
        	\label{fig:vis_nb201_c10}
         }
         \subfigure[CIFAR-100]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_cifar100.pdf}
        	\label{fig:vis_nb201_c100}
         }
         \subfigure[Aircraft]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_aircraft.pdf}
        	\label{fig:vis_nb201_aircraft}        
         }
         \subfigure[Oxford-IIIT Pets]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_pets.pdf}
        	\label{fig:vis_nb201_pets}        
         }
	% \vspace{-0.15in}
	\caption{\small \textbf{Architecture details in the MobileNetV3 search space.} We generate 5000 architectures and select 35 architectures using the dataset-aware surrogate model. Among these selected architectures, we provide the details of the architectures that achieve a top-5 accuracy for each dataset.}
	\label{fig:vis_nb201}
	\vspace{-0.15in}
\end{figure}

==> Figure_Tex/vis/nasbench201.tex <==
\begin{figure}[t]
	\centering
	% \vspace{-0.1in}
         \subfigure[CIFAR-10]{
        	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_cifar10.pdf}
        	\label{fig:vis_nb201_c10}
         }
         \subfigure[CIFAR-100]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_cifar100.pdf}
        	\label{fig:vis_nb201_c100}
         }
         \subfigure[Aircraft]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_aircraft.pdf}
        	\label{fig:vis_nb201_aircraft}        
         }
         \subfigure[Oxford-IIIT Pets]{
	\includegraphics[width=0.95\textwidth]{Figure/vis/vis_arch_pets.pdf}
        	\label{fig:vis_nb201_pets}        
         }
	% \vspace{-0.15in}
	\caption{\small \textbf{Architecture Details in the NAS-Bench-201 Search Space.} We generate 500 architectures and select 30 architectures using the dataset-aware surrogate model. Among these selected architectures, we provide the details of the architectures that achieve a top-5 accuracy for each dataset. 
    Furthermore, we present the average accuracy for each dataset below the architecture structure, which is computed from 3 different seeds.}
	\label{fig:vis_nb201}
	\vspace{-0.15in}
\end{figure}

==> Table/tbl_diffusion_vun.tex <==
% \begin{table*}[t!]
%     \caption{\small \textbf{Generation results on the NAS-Bench-201 and MobileNetV3 search spaces.} Best results are highlighted in bold.}
% \vspace{-0.1in}
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llccc}
%     \toprule
%         & \multirow{1}{*}{Method} & \multirow{1}{*}{Validity (\%) $\uparrow$} & \multirow{1}{*}{Uniqueness (\%) $\uparrow$} & \multirow{1}{*}{Novelty (\%) $\uparrow$} \\
%     \midrule
%         \multirow{5}{*}{NAS-Bench-201}
%         & EDP-GNN~\cite{shi2020graphaf} & xx.xx & xx.xx & xx.xx \\
%         & GDSS  & xx.xx & xx.xx & xx.xx \\
%         & DiGress~\cite{luo2021graphdf} & xx.xx & xx.xx & xx.xx \\
%         & Ours (w.o./ Pos. Emb.)~\cite{luo2021graphdf} & xx.xx & xx.xx & xx.xx \\
%         & Ours (w/ Pos. Emb.)  & xx.xx & xx.xx & xx.xx \\
%     \midrule
%     \multirow{5}{*}{MobileNetV3}
%         & EDP-GNN~\cite{shi2020graphaf} & xx.xx & xx.xx & xx.xx \\
%         & GDSS  & xx.xx & xx.xx & xx.xx \\
%         & DiGress~\cite{luo2021graphdf} & xx.xx & xx.xx & xx.xx \\
%         & Ours (w.o./ Pos. Emb.)~\cite{luo2021graphdf} & xx.xx & xx.xx & xx.xx \\
%         & Ours (w/ Pos. Emb.)  & xx.xx & xx.xx & xx.xx \\
%     \bottomrule
%     \end{tabular}}
%     \label{tab:diffusion_vun}
% \vspace{0.05in}
% \end{table*}

\begin{table*}[t!]{
\caption{\textbf{Generation results on the NAS-Bench-201 and MobileNetV3 search space.} Results are the means and the standard deviations of 3 runs.}
\label{tab:diffusion_vun}
\resizebox{\linewidth}{!}{
\renewcommand{\arraystretch}{1.0}
\renewcommand{\tabcolsep}{7pt}
\begin{tabular}{l c c c c c c} 
\toprule
\centering
    & \multicolumn{3}{c}{NAS-Bench-201} & \multicolumn{3}{c}{MobileNetV3} \\
\cmidrule(l{2pt}r{2pt}){2-4}
\cmidrule(l{2pt}r{2pt}){5-7}
    Method & Validity (\%) $\uparrow$ & Uniqueness (\%) $\uparrow$ & Novelty (\%) $\uparrow$ & Validity (\%) $\uparrow$ &  Uniqueness (\%) $\uparrow$ & Novelty (\%) $\uparrow$ \\
\midrule
    % EDP-GNN~\cite{niu2020permutation} &  xx.xx & xx.xx & xx.xx & xx.xx & xx.xx & xx.xx \\
    % GDSS~\cite{jo22GDSS} & 4.70 & 100.00 & 44.68 & xx.xx & xx.xx & xx.xx \\
    GDSS~\cite{jo22GDSS} &
    0.00\tiny$\pm$0.00 &
    - &
    - &
    0.00\tiny$\pm$0.00 &
    - &
    - \\
    % DiGress~\cite{vignac2022digress} &
    % xx.xx &
    % xx.xx &
    % xx.xx &
    % xx.xx &
    % xx.xx &
    % xx.xx \\
    Ours (w/o Pos. Emb.) & 
    \textbf{100.00\tiny$\pm$0.00} & 
    96.50\tiny$\pm$0.24 & 
    \textbf{49.33\tiny$\pm$1.06} & 
    16.63\tiny$\pm$0.74 &
    \textbf{100.00\tiny$\pm$0.00}&
    \textbf{100.00\tiny$\pm$0.00} \\
    Ours (w/ Pos. Emb.) & 
    \textbf{100.00\tiny$\pm$0.00} & 
    \textbf{96.53\tiny$\pm$0.41} & 
    48.17\tiny$\pm$1.05 & 
    \textbf{99.87\tiny$\pm$0.05} &
    \textbf{100.00\tiny$\pm$0.00} &
    \textbf{100.00\tiny$\pm$0.00} \\
\bottomrule
\end{tabular}
}
}\end{table*}

% sigma max = 5. / 1000개
% PC ()

==> Table/tbl_gen_dist.tex <==
\begin{wraptable}{r}{0.4\textwidth}
% \vspace{-0.15in}
\caption{\small Comparison between generators}\label{tbl:gen_dist}
% \vspace{-0.2in}
\resizebox{1.\linewidth}{!}{
\begin{tabular}{c|l|cccccc}
\toprule  
\small
Target & 
\multirow{2}{*}{Stats.} &
% \multirow{2}{*}{Oracle} & 
Oracle &
\multirow{2}{*}{Random} & 
\multirow{2}{*}{MetaD2A} &
Uncond. & 
Cond. &
Training \\
Dataset & 
&
Top-$1000$ &
& 
& 
+ Sorting. & 
(Ours) &
Dataset \\

\midrule
\midrule
\multirow{3}{*}{CIFAR10} &
Max &
94.3733 &
\textbf{94.3733} &
\textbf{94.3733} &
\textbf{94.3733} &
\textbf{94.3733} \\
xx.xx \\

&
Mean &
93.50 &
87.1169 &
91.5168 &
90.7705 &
\textbf{93.13} \\

&
Min &
93.18 &
10.0000 &
10.0000 &
10.0000 &
\textbf{86.44} \\

\midrule
\multirow{3}{*}{CIFAR100} &
Max &
\textbf{73.5133} &
72.7467 &
\textbf{73.5133} &
73.1667 &
\textbf{73.5133} \\

&
Mean &
xx.xx &
61.5902 &
67.1451 &
66.3792 &
\textbf{68.7529} \\

&
Min &
xx.xx &
1.0000 &
1.0000 &
1.0000 &
\textbf{44.1733} \\

\bottomrule
\vspace{-0.3in}
\end{tabular}
}
\end{wraptable} 

==> Table/tbl_main_nasbench201_old.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Performance on Unseen Datasets (Meta-Test)} MetaD2A conducts amortized inference on unseen target datasets after meta-training on source database consisting of subsets of ImageNet-1K and architectures of NAS-Bench-201 search space. Meta-training time is 12.7/8.4 GPU hours for the generator/the predictor. For fair comparison, the parameters of searched architectures are trained on each dataset from scratch instead of transferring parameters from ImageNet. $T$ is the time to construct precomputed architecture database for each target. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{clc|ccccc}
	   	\toprule
	   	\multirow{2}{*}{Target Dataset}             & 
	   	\multicolumn{1}{c}{\multirow{2}{*}{NAS Method}} & 
	   	Transfer                           &
	   	Params                                      & 
	   	Search Time                                 & 
	   	\multirow{2}{*}{Speed Up}                   &
	    Search Cost                                 & 
	   	Accuracy                                   \\ 
	   	                                            & 
	   	                                            & 
	   	NAS Method                                   & 
	   	(M)                                         & 
	   	(GPU Sec)                                   & 
	   	                                            & 
        (\$)                                        & 
	   	(\%)                                        \\
	   	\midrule
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   CIFAR-10  %%%%%%%%%%%%%%%%%%%%%%%%%
            \multirow{12}{*}{CIFAR-10}                 &
	   	ResNet~\citep{He16}                        &
	   	                                           &
	   	0.86                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	93.97\tiny$\pm$0.00                                      \\
	   	                                           &
	    REA~\citep{real2019regularized}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	0.02$+T$                                   & 
	   	-                                          &
	   	-                                          &
	   	93.92\tiny$\pm$0.30                        \\
	   	                                           &
	    RS~\citep{bergstra2012random}
	   	                                           &
	   	                                           &
	   	-                                          & 
	   	0.01$+T$                                   &         
	   	-                                          &  
	   	-                                          &
	    93.70\tiny$\pm$0.36                                                                             \\
	   	                                           &
	   REINFORCE~\citep{williams1992simple}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	0.12$+T$                                   & 
	   	-                                          &
	   	-                                          &
	    93.85\tiny$\pm$0.37                        \\
	   	                                           &
	   BOHB~\citep{falkner2018bohb}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	3.59$+T$                                   & 
	   	-                                          &
	   	-                                          &
	   	93.61\tiny$\pm$0.52                        \\
	   	\cdashline{2-8}                  
	   	                                           &
            GP-UCB                                     &
	   	                                        &
	   	-                                          &
	   	10200                                      &
	    147$\times$                                &
	   	4.13	   		   	                       &
	   	84.07\tiny$\pm$3.61                        \\
	   	                                           & 
            BANANAS~\citep{white2019bananas}                                     &
	   	                                        &
	   	-                                          &
	   	10200                                      &
	    147$\times$                                &
	   	4.13	   		   	                       &
	   	84.07\tiny$\pm$3.61                        \\
	   	                                           & 
            NASBOWL~\citep{ru2020interpretable}                                     &
	   	                                        &
	   	-                                          &
	   	10200                                      &
	    147$\times$                                &
	   	4.13	   		   	                       &
	   	84.07\tiny$\pm$3.61                        \\
	   	                                           & 
            HEBO~\citep{cowen2020hebo}                                     &
	   	                                        &
	   	-                                          &
	   	10200                                      &
	    147$\times$                                &
	   	4.13	   		   	                       &
	   	84.07\tiny$\pm$3.61                        \\
            \cdashline{2-8}
	   	                                           & 
            RSPS~\citep{li2020random}                  &
	   	                                           &
	   	-                                          &
	   	10200                                      &
	    147$\times$                                &
	   	4.13	   		   	                       &
	   	84.07\tiny$\pm$3.61                        \\
	   	                                           & 
	   	SETN~\citep{dong2019one}                   &
	   	                                           &
	   	-                                          &
	   	30200                                      &
	   	437$\times$                               &
	   	12.25	   		   	                       &
	   	87.64\tiny$\pm$0.00                        \\
	   	                                           & 
	   	GDAS~\citep{dong2019searching}             &
	   	                                           &
	   	-                                          &
	   	25077                                      &
	   	363$\times$                               &
	   	10.17	   		   	                       &
	   	93.61\tiny$\pm$0.09                        \\
	   	                                           & 
	   	PC-DARTS~\citep{xu2020pc}                  &
	   	                                           &
	   	1.17                                       &
	   	10395                                      &
	   	150$\times$                                &
	   	4.21	   		   	                       &
	   	93.66\tiny$\pm$0.17                       \\
	   	&
	   	DrNAS~\citep{chen2021drnas}                &
	   	                                           &
	   	1.53                                       &
	   	21760                                      &
	    315$\times$                                &
	    8.82	   		   	                       &
	   	94.36\tiny$\pm$0.00                        \\	   	
            \cdashline{2-8}
	   	                                           &
	   	MetaD2A~\citep{lee2021rapid}                 &
	   	\checkmark                                 &
	   	1.11                                        &
	   	\textbf{69}                                 &
	   	1$\times$                                  &
	   	\textbf{0.028}	   		   	               &
	   	\textbf{94.37\tiny$\pm$0.03}               \\
                                                 &
            TNAS~\citep{shalatransfer}                 &
	   	\checkmark                                 &
	   	1.11                                        &
	   	\textbf{69}                                 &
	   	1$\times$                                  &
	   	\textbf{0.028}	   		   	               &
	   	\textbf{94.37\tiny$\pm$0.03}               \\
                                                 &
            Ours                   &
	   	\checkmark                                 &
	   	1.07                                       &
	   	\textbf{96}                                &
	   	1$\times$                                  &
	   	\textbf{0.039}	   		   	               &
	   	\textbf{94.37\tiny$\pm$0.03}              \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   CIFAR-100  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{12}{*}{CIFAR-100}                 &
	   	ResNet~\citep{He16}                        &
	   	                                           &
	   	0.86                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	70.86\tiny$\pm$0.00                       \\
	   	                                           &
	    REA~\citep{real2019regularized}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	0.02+T                                          &
	   	-                                          &
        -                                          &
	   	71.84\tiny$\pm$0.99                       \\
	   	                                           &
	    RS~\citep{bergstra2012random}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	0.01+T                                          &
	   	-                                          &
	   	-                                          &
	   	71.04\tiny$\pm$1.07                        \\
	   	                                           &
	   REINFORCE~\citep{williams1992simple}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	0.12+T                                          &
	   	-                                          &
	   	-                                          &
	   	71.71\tiny$\pm$1.09                        \\
	   	                                           &
	   BOHB~\citep{falkner2018bohb}
	   	                                           &
	   	                                           &
	   	-                                          &
	   	3.59+T                                          &
	   	-                                          &
	   	-                                          &
	   	70.85\tiny$\pm$1.28                        \\
	   	\cdashline{2-8}                  
	   	                                           &
	   	RSPS~\citep{li2020random}                  &
	   	                                           &
	   	-                                          &
	   	18841                                      &
	   	196$\times$                                &
	   	7.64	   		   	                       &
	   	52.31\tiny$\pm$5.77                        \\
	   	                                           & 
	   	SETN~\citep{dong2019one}                   &
	   	                                           &
	   	-                                          &
	   	58808                                      &
	   	612$\times$                                &
	   	23.85	   		   	                       &
	   	59.09\tiny$\pm$0.24                       \\
	   	                                           & 
	   	GDAS~\citep{dong2019searching}             &
	   	                                           &
	   	-                                          &
	   	51580                                      &
	   	537$\times$                                &
	   	20.91	   		   	                       &
	   	70.70\tiny$\pm$0.30                        \\
	   	                                           & 
	   	PC-DARTS~\citep{xu2020pc}                  &
	   	                                           &
	   	0.26                                       &
	   	19951                                      &
	   	207$\times$                                &
	   	8.09	   		   	                       &
	   	66.64\tiny$\pm$2.34                        \\
	   	&
	   	DrNAS~\citep{chen2021drnas}                &
	   	                                           &
	   	1.20                                       &
	   	34529                                      &
	    359$\times$                                &
	    14.00                                      &
	   	\textbf{73.51\tiny$\pm$0.00}               \\	   	
	   	                                           &
	   	MetaD2A                   &
	   	\checkmark                                 &
	   	1.07                                       &
	   	\textbf{96}                                &
	   	1$\times$                                  &
	   	\textbf{0.039}	   		   	               &
	   	\textbf{73.51\tiny$\pm$0.00}               \\
                                                        &
            Ours                   &
	   	\checkmark                                 &
	   	1.07                                       &
	   	\textbf{96}                                &
	   	1$\times$                                  &
	   	\textbf{0.039}	   		   	               &
	   	\textbf{73.51\tiny$\pm$0.00}               \\
	   	\midrule
%%%%%%%%%%%%%%%%%%%%%%%%   Aircraft  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{8}{*}{Aircraft}                  &
	   	ResNet~\citep{He16}                        &
	   	                                           &
	   	0.86                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	47.01\tiny$\pm$1.16                                      \\
	   	                                           &
	   	RSPS~\citep{li2020random}                  &
	   	                                           &
	   	0.22                                       &
	   	18697                                      &
	   	1869$\times$                                &
	   	7.58	   		   	                       &
	   	42.19\tiny$\pm$3.88                        \\
	   	                                           & 
	   	SETN~\citep{dong2019one}                   &
	   	                                           &
	   	0.44                                       &
	   	18564                                      &
	   	1856$\times$                                &
	   	7.52	   		   	                       &
	   	44.84\tiny$\pm$3.96                       \\
	   	                                           & 
	   	GDAS~\citep{dong2019searching}             &
	   	                                           &
	   	0.62                                       &
	   	18508                                      &
	   	1850$\times$                                &
	   	7.50	   		   	                       &
	   	53.52\tiny$\pm$0.48                        \\
	   	                                           & 
	   	PC-DARTS~\citep{xu2020pc}                  &
	   	                                           &
	   	0.32                                       &
	   	3524                                        &
	   	352$\times$                                &
	   	1.42	   		   	                       &
	   	26.33\tiny$\pm$3.40                        \\
	   	&
	   	DrNAS~\citep{chen2021drnas}                &
	   	                                           &
	   	1.03                                       &
	   	34529                                      &
	    3452$\times$                                &
	    13.14	   		   	                       &
	   	46.08\tiny$\pm$7.00                        \\	   	
	   	                                           &
	   	MetaD2A                 &
	   	\checkmark                                 &
	   	0.83                                       &
	   	\textbf{10}                                &
	   	1$\times$                                  &
	   	\textbf{0.004}	   		   	               &
	   	58.43\tiny$\pm$1.18              \\
                                                 &
            Ours                   &
	   	\checkmark                                 &
	   	1.07                                       &
	   	\textbf{96}                                &
	   	1$\times$                                  &
	   	\textbf{0.039}	   		   	               &
	   	\textbf{58.79\tiny$\pm$0.54}  \\ %noise-T, r0.4        
	    \midrule
%%%%%%%%%%%%%%%%%%%%%%%%   Pets  %%%%%%%%%%%%%%%%%%%%%%%%%
	   	\multirow{8}{*}{Oxford-IIIT Pets}           &
	   	ResNet~\citep{He16}                        &
	   	                                           &
	   	0.86                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	N/A                                       &
	   	25.58\tiny$\pm$3.43                                      \\
	   	                                                      &
	   	RSPS~\citep{li2020random}                  &
	   	                                           &
	   	0.32                                       &
	   	3360                                       &
	   	420$\times$                                 &
	   	1.36	   		   	                       &
	   	22.91\tiny$\pm$1.65                        \\
	   	                                           & 
	   	SETN~\citep{dong2019one}                   &
	   	                                           &
	   	0.32                                       &
	   	8625                                       &
	   	1078$\times$                                &
	   	3.49	   		   	                       &
	   	25.17\tiny$\pm$1.68                       \\
	   	                                           & 
	   	GDAS~\citep{dong2019searching}             &
	   	                                           &
	   	0.83                                       &
	   	6965                                       &
	   	870$\times$                                &
	   	2.82	   		   	                       &
	   	24.02\tiny$\pm$2.75                        \\
	   	                                           & 
	   	PC-DARTS~\citep{xu2020pc}                  &
	   	                                           &
	   	0.44                                       &
	   	2844                                       &
	   	355$\times$                                 &
	   	1.15	   		   	                       &
	   	25.31\tiny$\pm$1.38                        \\
	   	&
	   	DrNAS~\citep{chen2021drnas}                &
	   	                                           &
	   	0.44                                       &
	   	6019                                       &
	    752$\times$                                &
	    2.44	   		   	                       &
	   	26.73\tiny$\pm$2.61                        \\	
	   	                                           &
	   	MetaD2A                   &
	   	\checkmark                                 &
	   	0.83                                       &
	   	\textbf{8}                                 &
	   	1$\times$                                  &
	   	\textbf{0.003}	   		   	               &
	   	\textbf{41.50\tiny$\pm$4.39}               \\
                                                 &
            Ours                   &
	   	\checkmark                                 &
	   	1.07                                       &
	   	\textbf{96}                                &
	   	1$\times$                                  &
	   	\textbf{0.039}	   		   	               &
	   	41.14\tiny$\pm$6.18  \\ %noise-T, r0.3              
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:main_nasbench201}
	\vspace{-0.15in}
	
\end{table*}


==> Table/tbl_main_nasbench201_time.tex <==
\begin{table*}[t!]
	\caption{\small \textbf{Performance on Unseen Datasets} NAS-Bench-201 search space. We report accuracies with $95\%$ confidence intervals. } %  45797/30152 GPU seconds
	\vspace{-0.15in}
	\small
	\begin{center}
     \resizebox{\linewidth}{!}{
	    \begin{tabular}{clcccccccc}
	   	\toprule
	   	\multicolumn{1}{c}{\multirow{3}{*}{Type}} & 
            \multicolumn{1}{c}{\multirow{3}{*}{Method}} &
            % \multicolumn{8}{c}{Target Dataset} & \\
            % &
            % &
            \multicolumn{2}{c}{CIFAR-10} &
            \multicolumn{2}{c}{CIFAR-100} &
            \multicolumn{2}{c}{Aircraft} &
            \multicolumn{2}{c}{Oxford-IIIT Pets} \\
            &
            &
            Accuracy &
            Trained &
            Accuracy &
            Trained &
            Accuracy &
            Trained &
            Accuracy &
            Trained \\
            &
            &
            (\%) &
            Models &
            (\%) &
            Models &
            (\%) &
            Models &
            (\%) &
            Models \\
            \midrule
	   	\midrule
            % &
            % Random &
            % 93.42\tiny$\pm$0.34 &
            % xx.xx &
            % \textbf{73.51\tiny$\pm$0.00} &
            % xx.xx &
            % 35.62\tiny$\pm$4.75 &
            % xx.xx &
            % 29.40\tiny$\pm$2.07 &
            % xx.xx \\
            &
            ResNet~\citep{He16} &
            93.97\tiny$\pm$0.00 &
            N/A &
            70.86\tiny$\pm$0.00 &
            N/A &
            47.01\tiny$\pm$1.16 &
            N/A &
            25.58\tiny$\pm$3.43 &
            N/A \\
            &
            RS~\citep{bergstra2012random} &
            93.70\tiny$\pm$0.36 &
            0.01$+T$ &
            71.04\tiny$\pm$1.07 &
            0.01$+T$ &
            - &
            - &
            - &
            - \\
            &
            REA~\citep{real2019regularized} &
            93.92\tiny$\pm$0.30 &
            0.02$+T$ &
            71.84\tiny$\pm$0.99 &
            0.02$+T$ &
            - &
            - &
            - &
            - \\
            &
            REINFORCE~\citep{williams1992simple} &
            93.85\tiny$\pm$0.37 &
            0.12$+T$ &
            71.71\tiny$\pm$1.09 &
            0.12$+T$ &
            - &
            - &
            - &
            - \\
            &
            RSPS~\citep{li2020random} &
            84.07\tiny$\pm$3.61 &
            10200 &
            52.31\tiny$\pm$5.77 &
            18841 &
            42.19\tiny$\pm$3.88 &
            18697 &
            22.91\tiny$\pm$1.65 &
            3360 \\
            %\cdashline{1-10}
            \midrule
            \multicolumn{1}{c}{\multirow{4}{*}{One-shot NAS}} &
            SETN~\citep{dong2019one} &
            87.64\tiny$\pm$0.00 &
            30200 &
            59.09\tiny$\pm$0.24 &
            58808 &
            44.84\tiny$\pm$3.96 &
            18564 &
            25.17\tiny$\pm$1.68 &
            8625 \\
            &
            GDAS~\citep{dong2019searching} &
            93.61\tiny$\pm$0.09 &
            25077 &
            70.70\tiny$\pm$0.30 &
            51580 &
            53.52\tiny$\pm$0.48 &
            18508 &
            24.02\tiny$\pm$2.75 &
            6965 \\
            &
            PC-DARTS~\citep{xu2020pc} &
            93.66\tiny$\pm$0.17 &
            10395 &
            66.64\tiny$\pm$2.34 &
            19951 &
            26.33\tiny$\pm$3.40 &
            3524 &
            25.31\tiny$\pm$1.38 &
            2844 \\
            &
            DrNAS~\citep{chen2021drnas} &
            94.36\tiny$\pm$0.00 &
            21760 &
            \textbf{73.51\tiny$\pm$0.00} &
            34529 &
            46.08\tiny$\pm$7.00  &
            34529 &
            26.73\tiny$\pm$2.61 &
            6019 \\
            %\cdashline{1-10}
            \midrule
            % \multirow{5}{*}{\rotatebox[origin=c]{90}{\small BO-based NAS}} 
            \multicolumn{1}{c}{\multirow{5}{*}{BO NAS}} &
            BOHB~\citep{falkner2018bohb} &
            93.61\tiny$\pm$0.52 &
            3.59$+T$ &
            70.85\tiny$\pm$1.28 &
            3.59$+T$ &
            - &
            - &
            - &
            - \\
            &
            GP-UCB &
            \textbf{94.37\tiny$\pm$0.00} &
            xx.xx &
            73.14\tiny$\pm$0.00 &
            xx.xx &
            41.72\tiny$\pm$0.00 &
            xx.xx &
            % 41.98\tiny$\pm$0.00 &
            40.60\tiny$\pm$0.00 &
            xx.xx \\
            &
            BANANAS~\citep{white2019bananas} &
            \textbf{94.37\tiny$\pm$0.00} &
            xx.xx &
            \textbf{73.51\tiny$\pm$0.00} &
            xx.xx &
            41.72\tiny$\pm$0.00 &
            xx.xx &
            % 41.29\tiny$\pm$1.10 &
            40.15\tiny$\pm$1.10 &
            xx.xx \\
            &
            NASBOWL~\citep{ru2020interpretable} &
            94.34\tiny$\pm$0.00 &
            xx.xx &
            \textbf{73.51\tiny$\pm$0.00} &
            xx.xx &
            53.73\tiny$\pm$0.83 &
            xx.xx &
            % 41.98\tiny$\pm$0.00 &
            41.29\tiny$\pm$0.00 &
            xx.xx \\
            &
            HEBO~\citep{cowen2020hebo} &
            94.34\tiny$\pm$0.00 &
            xx.xx &
            72.62\tiny$\pm$0.20 &
            xx.xx &
            49.32\tiny$\pm$6.10 &
            xx.xx &
            40.55\tiny$\pm$1.15 &
            xx.xx \\
            %\cdashline{1-10}
            \midrule
            % \multirow{5}{*}{\rotatebox[origin=c]{90}{\small Transfer NAS}} 
            \multicolumn{1}{c}{\multirow{3}{*}{TransferNAS}} &
            MetaD2A~\citep{lee2021rapid} &
            \textbf{94.37\tiny$\pm$0.00} &
            xx.xx &
            73.34\tiny$\pm$0.04 &
            xx.xx &
            57.71\tiny$\pm$0.20 &
            xx.xx &
            39.04\tiny$\pm$0.20 &
            xx.xx \\
             &
            TNAS~\citep{shalatransfer} &
            \textbf{94.37\tiny$\pm$0.00} &
            xx.xx &
            \textbf{73.51\tiny$\pm$0.00} &
            xx.xx &
            59.51\tiny$\pm$0.00 &
            xx.xx &
            % 43.24\tiny$\pm$0.00 &
            40.00\tiny$\pm$0.00 &
            xx.xx \\
             &
            Ours &
            \textbf{94.37\tiny$\pm$0.00} &
            xx.xx &
            \textbf{73.51\tiny$\pm$0.00} &
            xx.xx &
            \textbf{59.63\tiny$\pm$0.00} &
            xx.xx &
            \textbf{41.80\tiny$\pm$0.00} &
            xx.xx \\
            % &
            % Ours &
            % \textbf{94.37\tiny$\pm$0.00} &
            % xx.xx &
            % \textbf{73.51\tiny$\pm$0.00} &
            % xx.xx &
            % \textbf{59.63} &
            % xx.xx &
            % xx.xx &
            % xx.xx \\
            
	   	\bottomrule
        \end{tabular}
	    }
	\end{center}
	\small
	\label{tbl:main_nasbench201}
	\vspace{-0.15in}
	
\end{table*}



==> Table/tbl_suppl_guidance.tex <==

\begin{table}[t!]
\caption{\small \textbf{Validity Results - Coarse Grid Search} }
\vspace{-0.1in}
\tiny
\begin{center}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
Guidance Strength  & $10^6$     & $10^5$ & \textbf{$10^4$} \\
                           
\midrule
\midrule
Validity                 & 0.0               & 0.0 & \textbf{100.0}   \\
\bottomrule
\end{tabular}
} 	
\end{center}
\label{tbl:suppl_guidance}
\vspace{-0.15in}
\end{table}


==> Table/tbl_suppl_guidance_abl.tex <==

\begin{table}[t!]
\caption{\small \textbf{Ablation Study - Guidance Strength} Distribution of generated neural architectures across various sampling strategies. All methods generated neural architectures within the same sampling time. }
\vspace{-0.1in}
\tiny
\begin{center}
\resizebox{1.0\linewidth}{!}{
% {\color{blue}\begin{tabular}{cccc}
% \toprule
% Stats.  & Fixed at a large value    & Balanced exploitation-exploration  
% (Ours) & Fixed at a small value  \\
                           
% \midrule
% \midrule
% Max Accuracy (\%)                                   & 94.3633 & \textbf{94.3733} & \textbf{94.3733} \\ 
% Mean Accuracy (\%)                                  & 93.4658 & 93.1881 & 93.0640 \\ 
% Min Accuracy (\%)                                   & 90.6450 & 89.9367 & 88.1767 \\ 
% Standard Deviation (\%)                             & 1.0334  & 1.2118  & 1.4169  \\ 
% Avg. Acc. of Top-5 (\%) & 93.9880 & \textbf{94.2477} & 93.8833 \\
% \bottomrule
% \end{tabular}
% } 	
\begin{tabular}{cccc}
\toprule
Stats.  & Fixed at a large value    & Balanced exploitation-exploration  
(Ours) & Fixed at a small value  \\
                           
\midrule
\midrule
Avg. Acc. of Top-5 (\%) & 93.262 & \textbf{94.156} & 93.978 \\
Standard Deviation (\%)                             & 0.395 & 0.658 & 0.953  \\ 
\bottomrule
\end{tabular}
} 	

\end{center}
\label{tbl:suppl_guidance_abl}
\vspace{-0.15in}
\end{table}


==> Table/tbl_top_dist.tex <==
\begin{table}[t]{
\centering
\caption{\small \textbf{Top 1\% results.} \small Results}
\label{tbl:top_dist}
% \vspace{-0.15in}
	\small
	\begin{center}
        % \resizebox{\columnwidth}{!}{
        \resizebox{\linewidth}{!}{
        \begin{tabular}{ccccccc}
        \toprule
\multirow{Method} 
& \multicolumn{6}{c}{Target Dataset} \\ \cline{2-7} 
& \multicolumn{2}{c}{CIFAR-10} 
& \multicolumn{2}{c}{CIFAR-100} 
& \multicolumn{2}{c}{ImageNet16-120} \\ \cline{2-7} 
& ACC           & LAT          & ACC           & LAT           & ACC              & LAT          \\ \midrule
No-Gui.           & xx.xx         & xx.xx        & xx.xx         & xx.xx         & xx.xx            & xx.xx           \\ \midrule 
ACC-Gui. ($k_t=0.5$)          & xx.xx         & xx.xx        & xx.xx         & xx.xx         & xx.xx            & xx.xx           \\ \midrule 
ACC-Gui. ($k_t=1.0$)            & xx.xx         & xx.xx        & xx.xx         & xx.xx         & xx.xx            & xx.xx           \\ \midrule
LAT-Gui. ($k_t=0.5$)          & xx.xx         & xx.xx        & xx.xx         & xx.xx         & xx.xx            & xx.xx           \\ \midrule 
LAT-Gui. ($k_t=1.0$)            & xx.xx         & xx.xx        & xx.xx         & xx.xx         & xx.xx            & xx.xx           \\ \bottomrule 


\end{tabular}
	    }
	\end{center}
	\small
	% \vspace{-0.15in}
\end{table}

==> Table/tbl_uniquness.tex <==
\begin{table}
\begin{minipage}{.495\textwidth}
    \caption{\textbf{Uniqueness}
    }
\centering
\caption{\small \textbf{Uniqeness.} \small Results}
\label{tbl:uniqueness}
\begin{tabular}{ll}
% \vspace{-0.15in}
\small
% \begin{center}
    % \resizebox{1.0\columnwidth}{!}{
    % \begin{tabular}{ccccccccc}
    \toprule
\multirow{Method} 
& \multicolumn{8}{c}{Target Dataset} \\ \cline{2-7} 
& \multicolumn{3}{c}{CIFAR-10} 
& \multicolumn{3}{c}{CIFAR-100} 
& \multicolumn{3}{c}{ImageNet16-120} \\ \cline{2-7} 
& ACC           
& LAT
& Uniqueness
& ACC           
& LAT    
& Uniqueness
& ACC              
& LAT       
& Uniqueness
\\ \midrule
No-Gui.           
& xx.xx         
& xx.xx        
& xx.xx         
& xx.xx    
& xx.xx        
& xx.xx         
& xx.xx 
& xx.xx            
& xx.xx           \\ \midrule 
ACC-Gui. ($k_t=0.5$)          
& xx.xx         
& xx.xx        
& xx.xx         
& xx.xx        
& xx.xx         
& xx.xx 
& xx.xx         
& xx.xx            
& xx.xx           \\ \midrule 
ACC-Gui. ($k_t=1.0$)            
& xx.xx         
& xx.xx        
& xx.xx         
& xx.xx         
& xx.xx        
& xx.xx         
& xx.xx 
& xx.xx            
& xx.xx           \\ \midrule
LAT-Gui. ($k_t=0.5$)          
& xx.xx         
& xx.xx        
& xx.xx        
& xx.xx        
& xx.xx         
& xx.xx 
& xx.xx         
& xx.xx            
& xx.xx           \\ \midrule 
LAT-Gui. ($k_t=1.0$)            
& xx.xx         
& xx.xx        
& xx.xx        
& xx.xx         
& xx.xx 
& xx.xx         
& xx.xx         
& xx.xx            
& xx.xx           \\ \bottomrule 


% \end{tabular}
	    % }
	% \end{center}
	\small
	% \vspace{-0.15in}
 \end{tabular}
\end{minipage}
\end{table}
